When Private Blockchain Meets Deterministic Database

Private blockchain as a replicated transactional system shares many commonalities with distributed database. However, the intimacy between private blockchain and deterministic database has never been studied. In essence, private blockchain and deterministic database both ensure replica consistency by determinism. In this paper, we present a comprehensive analysis to uncover the connections between private blockchain and deterministic database. While private blockchains have started to pursue deterministic transaction executions recently, deterministic databases have already studied deterministic concurrency control protocols for almost a decade. This motivates us to propose Harmony, a novel deterministic concurrency control protocol designed for blockchain use. We use Harmony to build a new relational blockchain, namely HarmonyBC, which features low abort rates, hotspot resiliency, and inter-block parallelism, all of which are especially important to disk-oriented blockchain. Empirical results on Smallbank, YCSB, and TPC-C show that HarmonyBC offers 2.0x to 3.5x throughput better than the state-of-the-art private blockchains.

==> background.tex <==
\section{Background} \label{background}
In this section,
we provide essential background 
on private blockchain and deterministic database.
A thorough discussion of related work is in 
Section \ref{sec:related}.

\subsection{Private Blockchain}
Recent private blockchains mainly have two architectures: Simulate-Order-Validate (SOV) and Execute-Order (EO).

\stitle{Simulate-Order-Validate (SOV)} is 
a blockchain execution framework 
advocated by Fabric \cite{fabric}.
Fabric's progeny such as FastFabric \cite{fastfabric},
Fabric++ \cite{fabric++} and Fabric\#\cite{fabricsharp} all follow the same architecture.
In SOV, clients submit transactions to a subset of
peers/replicas (known as \emph{endorsers}).
On arriving an endorser, 
a transaction begins its simulation phase 
and ``executes'' against the replica's \emph{latest state}
without applying any of its writes.
The purpose of the simulation phase is collect the read-write set of the transaction, where the read-set contains keys and version numbers for all read records and the write-set contains the updated keys and their new values.

The simulation of a transaction, however, is non-deterministic across replicas.
Specifically, inside an endorser, 
although the transactions within their simulation phases 
would not update the endorser's state,
that state would still be progressively updated by \emph{transactions from 
prior blocks} that already passed their validation phase.
As we will see next, the read-write sets 
passing the validation phase and the ordering of applying them 
are deterministic.
However, there are other sources of non-determinism for transactions in this stage.
For example, a client transaction may arrive different endorsers asynchronously.
Hence, the read-write sets simulated for the same client transaction may 
diverge across endorsers.
Due to the non-determinism, 
the SOV paradigm requires the endorsers 
to send the potential divergent read-write sets of the same transaction
back to the client who picks an agreed one for that transaction.
That is essentially a network round-trip cost paid
to resolve the non-determinism.

After simulation, a client sends the signed read-write set of a transaction 
to an ordering service.
The ordering service consolidates client transactions and forms transaction blocks based on the transaction arrival order.
After that, the ordering service broadcasts 
the block to all replicas.
The ordering step is deterministic.
However, a broadcasted block from an ordering service may 
still arrive the replicas asynchronously, 
especially under a wide-area network.

On receiving a transaction block,
a replica validates the security (e.g., verifying the signatures)
and the serializability of that block of transactions.
For the latter, a replica checks if the versions of the received read-set are consistent with the replica's local version, aborts the staled ones,
and commits the rest by applying the write-sets to its local state.



To reduce the number of aborted transactions
that violate serializability, 
Fabric++ \cite{fabric++} and Fabric\# \cite{fabricsharp} 
employs the ordering service to 
analyze the dependencies between the transactions within a block 
and reorder them in order to reduce the number of transactions that would 
fail the serializability check.
On receiving a block of (reordered) transactions,
a replica \emph{serially} applies the transactions to its local state to ensure replica consistency.




\stitle{Order-Execute (OE)} is the blockchain execution framework used by Bitcoin and 
recent private blockchains like RBC \cite{rbc} and ChainifyDB \cite{chainifydb}. 
In OE, clients submit transactions to an ordering service straight.
The job of the ordering service in OE is the same as in SOV --- 
collects client transactions, orders transactions with a particular order and forms blocks, and broadcasts blocks to the replicas. 
On receiving a block of transactions, 
each replica executes the block independently with a goal of 
reaching identical next states.

To uphold consistent across replicas, 
replicas shall execute the same block of transactions serially.
ChainifyDB and RBC, however, can do that with parallelism and concurrency.
In ChainifyDB,
each replica applies static analysis on the transactions of the block
to infer their read-write sets.
Then, each replica use the information of the 
read-write sets 
to devise a serializable schedule whose commit order honors 
the transaction order listed in the block.
Static analysis however has one limitation --- 
the exact read-write sets cannot be inferred a priori 
if there is any transactional logic that branches on query results.



RBC works without using static analysis.
After receiving a transaction block $i$ from an ordering service,
an RBC replica ``executes'' transactions in block $i$ against the replica's \emph{last block state} without applying any of its writes.
Notice the subtleties between SOV and OE here.
In SOV, a transaction is simulated against the \emph{latest} replica state (which is updatable by other transactions that are in the other stage of pipeline, i.e., the validation phase).  
In contrast, a transaction in OE is simulated against a static state
--- the state after executing the last block, i.e., block $i-1$.
Such a last block state $i-1$ is identical to all transactions in block $i$.
Hence, in OE,
a replica can ``executes'' all transactions of a block in parallel.
Furthermore, since all replicas processes 
the same block $i$ by referencing to 
the same and static $i-1$ state, the read-write sets of the transactions
are also consistent across replicas.
Hence, as long as every replica also follows the same order to 
\emph{serially} validates, aborts, and commits the read-write sets of a block,
RBC can achieve replica consistency.

RBC supports inter-block parallelism --- transactions from different blocks can be processed concurrently.
When that enabled,
a client $C$ who wants to submit a transaction $T$ first consults a replica $R$ about 
the block number of the replica's last completed block.
Assume there are 3 replicas $R_1$, $R_2$, and $R_3$, 
which have just finished blocks 10, 9, and 8, respectively (since replicas may have different processing speed)
and client $C$ gets to know that replica $R_2$ just finished block 9.
Since then, $C$ would regard the state right after block 9 as its reference state and 
broadcast $T$ to \emph{both} the ordering service \emph{and all replicas} 
with the block number 10 tagged along.
In the ordering service, $T$ will get ordered and form blocks with the other
received transactions as usual.
Let us assume the ordering service is busy and $T$ gets arranged into, say, block 14.
Meanwhile, all three replicas are processing $T$ as well.
On receiving a transaction $T$, 
a replica simulates $T$ against the state designated by the block number tagged along with the transaction to obtain its read-write set.
In our example, that is the state after block 9.
After simulation, 
the replica would not be validated and committed $T$
until the block containing $T$ formally arrived
from the ordering service.
The use of inter-block parallelism in RBC 
enables transaction executions (by replicas) 
and transaction ordering (by ordering service)
happen in parallel.
The trade-off is the potential increase of aborts 
because the time gap between 
a transaction ``execution'' and its validation would introduce a lot of stale reads.
In our example, when the transaction $T$ arrives a replica 
as part of block 14 after ordering, it would get aborted 
as long as any of its reads becomes stale if it conflicts with
any update from blocks 11 to 13.










\subsection{Deterministic Database}
A deterministic database typically contain a \emph{sequencing layer} and each replica hosts a \emph{transaction engine}.
The sequencing layer collects transactions from client application and assign a unique transaction ID (TID) to each transaction. The transactions are then broadcast to the replicas block-by-block.
When a block of transactions reaches a replica and the previous block is finished, 
the replica executes the transactions in parallel using 
a deterministic concurrency control scheme, and replicas reach the same state after executing the block.

Inside the transaction engine, Calvin uses \textit{deterministic two-phase-locking} to grant locks in a deterministic order.
Concretely, if two conflicting transactions intend to lock the same record, the one with a smaller TID gets the lock first (thus things are deterministic).
However, this cannot be done without the knowledge of all the read-write-sets of the transactions in the block before the execution.
Consider a transaction $T_5$ first requests a lock on record $x$ during execution. The lock manager cannot determine whether to grant the lock unless it knows whether all the transactions whose \texttt{TID}s $<$ 5 would access $x$ or not.  
Therefore, on receiving a block of transactions,
Calvin first (1) 
carries out static analysis to infer the read-write-sets.
Then, Calvin (2) 
devices a deterministic lock-granting order based on the read-write-sets and the TIDs.
Finally, Calvin (3) follows the lock-granting order to grant locks to the transactions, a transaction executes if it acquires necessary locks.
BOHM \cite{bohm} and PWV \cite{pwv} are similar to Calvin in which they all begin with static analysis.

The latest deterministic database Aria \cite{aria} addresses this limitation by \emph{deterministic optimistic concurrency control} (OCC).
Similar to optimistic concurrency control, its transaction engine run transactions in three steps: simulation, validation and commit.
It (1) first concurrently simulates the transactions of a block against the same snapshot --- the final state of the previous block, which is identical among all replicas. The identical read-write-sets are produced on all replicas and no write-sets are applied.
Afterwards, Aria starts (2) validation phase where it analyzes the read/write-dependencies from the read-write-sets 
to deterministically mark
transactions that violate serializability to abort.
Finally, it enters (3) the commit phase to apply the write-sets of the transactions to be committed, and then commit/abort transactions . 







